Minimally Entangled Typical Thermal States Algorithms for Finite Temperature Matsubara Green Functions

We extend finite-temperature tensor network methods to compute Matsubara imaginary-time correlation functions, building on the minimally entangled typical thermal states (METTS) and purification algorithms. While imaginary-time correlation functions are straightforward to formulate with these methods, care is needed to avoid convergence issues that would result from naive estimators. As a benchmark, we study the single-band Anderson impurity model, even though the algorithm is quite general and applies to lattice models. The special structure of the impurity model benchmark system and our choice of basis enable techniques such as reuse of high-probability METTS for increasing algorithm efficiency. The results are competitive with state-of-the-art continuous time Monte Carlo. We discuss the behavior of computation time and error as a function of the number of purified sites in the Hamiltonian.

==> OlderIntro.tex <==
STOPSTOPSTOPSTOP
The ultimate challenge in quantum many-body physics is to find ways how to deal with the exponentially growing state space that describes interacting quantum systems. One such way of taming the many-body complexity is the density matrix renormalization group (DMRG)~\cite{White_DMRG, SCHOLLWOCK201196} whose success is based on the celebrated area laws of entanglement~\cite{Eisert_AreaLaws}. These area laws effectively state that for one-dimensional, gapped quantum systems, matrix product states (MPS) are an efficient representation of its ground states. While MPS work very well for one-dimensional systems, its generalizations to higher dimensions is highly non-trivial and is still an active area of research \DB{Miles what are a couple of nice PEPS papers to cite here?}. 

Another strategy of dealing with the exponentially growing Hilbert spaces are sampling based quantum Monte Carlo (QMC) methods. Compared to classical Monte Carlo, QMC samples not only from $d$-dimensional space but, because of quantum effects, also from an additional imaginary time dimension and sampling is carried out in $d+1$ dimensions. While QMC is statistically exact, the imaginary time dimension can introduce a (negative) sign problem where convergence becomes exponentially costly with decreasing temperature.

A third strategy is to simplify the Hamiltonian itself, for example via mean-field approaches. Mean-field theories replace the original model by a simpler one that depends self consistently on its own solution. In dynamical mean field theory (DMFT)~\cite{Georges_DMFT,Metzner_DMFT} for example, a lattice model is replaced by an Anderson impurity model and the parameters of its bath are determined self-consistently. The approximation used to close the self-consistency loop is that of a local single particle self energy,  which becomes more accurate in higher dimensional systems and eventually becomes exact in the limit $d \to \infty$. The arguably \emph{simpler} impurity models are themselves complex many-body problems and require advanced methods like the numerical renormalization group (NRG)~\cite{NRG_bulla, NRG_original}, the above mentioned tensor networks~\cite{FTPS,Schollwoeck_ImagTimeSolver}, or QMC~\cite{CTHYB1, CTHYB2} to solve.

This requires the computation of a certain dynamical correlation function: the single-particle Green function. Apart from DMFT, dynamical correlation functions also play a central role in linear-response theory by describing the response of a system to an external perturbation. Therefore, the computation of correlation functions is of large interest in quantum many-body physics.

While QMC computes dynamical correlation functions mostly in imaginary time (see Ref.~\cite{Gull_RealTimeMC} for an exception \DB{add diagramatic MC?}), MPS based methods can perform the computation in real- as well as imaginary times. Apart from some notable exceptions~\cite{Schollwoeck_ImagTimeSolver,Schollwoeck_ImagTimeSolver_2,Zingl_ImagTimeSolver}, the focus of MPS-based methods so far was mostly on real-time evolutions. Even though the imaginary frequency axis makes it hard to resolve high-energy features, low energies are captured well and the zero energy limit is even exact. Additionally, imaginary time evolution ultimately always projects to ground states for which we already know that they can be represented well as a MPS. Comparing that to states evolved in real-time for which the MPS bond dimension grows fast (sometimes exponentially) shows that imaginary time evolution should be considered more often as a valid way to access low energy spectral information.

In this work, we present an approach that combines the ideas and strategies mentioned above. We use existing sign problem free finite temperature MPS methods based on sampling and compute imaginary time correlation functions. When applied to an Anderson impurity model, we find an extremely efficient\DB{wording!} approach that works very well even for samples of size $1$.

Finite temperature methods using MPS were usually categorized either into methods that compute the full thermal density matrix~\cite{Verstraete_purification} or the so-called minimally typical thermal states (METTS)~\cite{Miles_Metts} which is based on sampling. Only recently these two approaches were combined in a unifying framework allowing a smooth transition between the two methods~\cite{Jing_HybridPurificationMetts,chung_2019minimally}. In this work we hence adopt the viewpoint of purification as a METTS method in which no sampling at all is required. Both approaches integrate the imaginary time dimension exactly and the sampling then only need needs to be performed in the remaining $d$-dimensions. This is the reason why METTS does not suffer from a negative sign problem because all probabilities are diagonal entries of the thermal density matrix. While finite temperature correlation functions were computed previously, again, most of the focus was on real-time evolution via the purification~\cite{Purification_RT_Barthel,Purification_RT_Garst,Purification_RT_Meissner, Purification_RT_Karasch1, Purification_RT_Karasch2, Purification_RT_Karasch3,Purification_RT_Karasch4, Purification_RT_Karasch5, Purification_RT_Karasch6,Purification_RT_Karasch7, Purification_RT_Karasch8} or METTS~\cite{Metts_RT_Barthel,Metts_RT_Laeuchli, Metts_RT_Weichselbaum} and imaginary time correlators have not gotten a lot of attention.




% CONCLUSION



The computational cost of METTS, is to perform imaginary time evolution up to $\beta/2$ with $\beta$ the inverse temperature. Due to cancellations of the imaginary time evolution to compute the METTS itself and the correlation function, one ends up with a total of $3\beta/2$ total time evolution. This means that computing imaginary time correlation functions should in principle be possible for most models for which one can compute METTS. This would even open up the possibility to compute the low-energy part of response functions of 2d-like cylinder systems as for example shown for the Hubbard model in Ref.~\cite{wietek2020stripes}.



The rest of the paper is structured as follows. In Sec.~\ref{sec:METTS} we briefly introduce the original METTS algorithm as well as how to combine METTS and purification and define the estimator to sample imaginary time correlators. In Sec.~\ref{sec:ModelMethods} we introduce the Anderson Impurity models we focus on in the present work and also discuss computational parameters and methods. Results are presented in Sec.~\ref{sec:results} where we first discuss the choice of estimator to measure correlation functions and then discuss in detail the peculiar behavior that METTS shows when used for impurity models. 

